Assessing the techno-economic benefits of LEMs for different grid topologies and prosumer shares

The shift towards decentralized and renewable energy sources has introduced significant challenges to traditional power systems, necessitating innovative market designs. Local energy markets present a viable solution for integrating distributed energy resources such as photovoltaic systems, electric vehicles, and heat pumps within various grid topologies. This study investigates the techno-economic benefits of local energy markets compared to conventional market designs, focusing on their impact on average energy prices and operational peak power, using a self-developed agent-based energy system simulation tool. Through comprehensive simulations across the countryside, rural, suburban, and urban grid topologies with varying penetration levels of the distributed energy resources, totaling 400 simulation setups, we demonstrate that local energy markets can enhance economic efficiency and grid stability with 99 % of the scenarios boasting lower average energy prices and 80 % lower operational peak power levels. Our findings suggest that local energy markets can play a role in the future energy system, especially in areas with high shares of PV and HP, provided that additional infrastructure, management costs, and bureaucratic complexity are kept to a minimum.

==> sections/figures.tex <==

% introduction
\begin{figure}
    \centering
    \includegraphics[width=.8\textwidth]{figure/lem_combinations.png}
    \caption{Methodology for the creation of the scenarios to be examined}
    \label{fig:scenario_creation}
\end{figure}


    
% results/relative impact
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/Countryside_price_power_all_all.png}
        \caption{Countryside}
        \label{fig:price_power_countryside}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/Rural_price_power_all_all.png}
        \caption{Rural}
        \label{fig:price_power_rural}
    \end{subfigure}

    \vspace{1ex} % Adjust vertical spacing between the rows of subfigures

    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/Suburban_price_power_all_all.png}
        \caption{Suburban}
        \label{fig:price_power_suburban}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/Urban_price_power_all_all.png}
        \caption{Urban}
        \label{fig:price_power_urban}
    \end{subfigure}

    \caption{Comparison of the average energy price and operational peak power ratio for scenarios with and without LEMs for every combination of PV, EV and HP}
    \label{fig:price_power}
\end{figure}

% results/absolute price
\begin{figure}
    \centering
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figure/Countryside_price_all_all.png}
    %     \caption{Countryside}
    %     \label{fig:price_countryside}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/Rural_price_all_all.png}
        \caption{Rural}
        \label{fig:price_rural}
    \end{subfigure}
    % \vspace{1em} % Adjust vertical spacing between the rows of subfigures
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/Suburban_price_all_all.png}
        \caption{Suburban}
        \label{fig:price_suburban}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figure/Urban_price_all_all.png}
    %     \caption{Urban}
    %     \label{fig:price_urban}
    % \end{subfigure}

    \caption{Comparison of the absolute energy prices for scenarios with and without LEMs for every combination of PV, EV and HP}
    \label{fig:price}
\end{figure}


% results/absolute power
\begin{figure}
    \centering
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figure/Countryside_power_all_all.png}
    %     \caption{Countryside}
    %     \label{fig:power_countryside}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/Rural_power_all_all.png}
        \caption{Rural}
        \label{fig:power_rural}
    \end{subfigure}
    % \vspace{1em} % Adjust vertical spacing between the rows of subfigures
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/Suburban_power_all_all.png}
        \caption{Suburban}
        \label{fig:power_suburban}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figure/Urban_power_all_all.png}
    %     \caption{Urban}
    %     \label{fig:power_urban}
    % \end{subfigure}

    \caption{Comparison of the operational peak power values for scenarios with and without LEMs for every combination of PV, EV and HP}
    \label{fig:power}
\end{figure}


% results/in-depth
\begin{figure}
    \centering
    % \begin{subfigure}[b]{0.49\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figure/Countryside_power_all_all.png}
    %     \caption{Countryside}
    %     \label{fig:indepth_countryside}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/Rural_indepth.png}
        \caption{Rural}
        \label{fig:indepth_rural}
    \end{subfigure}
    % \vspace{1em} % Adjust vertical spacing between the rows of subfigures
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/Suburban_indepth.png}
        \caption{Suburban}
        \label{fig:indepth_suburban}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.49\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figure/Urban_power_all_all.png}
    %     \caption{Urban}
    %     \label{fig:indpeth_urban}
    % \end{subfigure}

    \caption{In-depth analysis of the effects under specific penetration rates of PV, EV and HP on the average energy price and the operational peak power values in LEMs}
    \label{fig:indepth}
\end{figure}

% discussion/implications
\begin{figure}
    \centering
    % Summer
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/summer_wolem.png}
        \caption{Summer -- without LEM}
        \label{fig:powerflow_summer_woLEM}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/summer_wlem.png}
        \caption{Summer -- with LEM}
        \label{fig:powerflow_summer_wLEM}
    \end{subfigure}

    \vspace{1em} % Adjust vertical spacing between the rows of subfigures
    
    % Transition
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/transition_wolem.png}
        \caption{Transition -- without LEM}
        \label{fig:powerflow_transition_woLEM}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/transition_wlem.png}
        \caption{Transition -- with LEM}
        \label{fig:powerflow_transition_wLEM}
    \end{subfigure}

    \vspace{1em} % Adjust vertical spacing between the rows of subfigures
    
    % Winter
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/winter_wolem.png}
        \caption{Winter -- without LEM}
        \label{fig:powerflow_winter_woLEM}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/winter_wlem.png}
        \caption{Winter -- with LEM}
        \label{fig:powerflow_winter_wLEM}
    \end{subfigure}

    \caption{Figure plotting the power flows of the system with and without LEM}
    \label{fig:powerflow}
\end{figure}

% methodology/market design
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figure/LEM_structure.png}
    \caption{The trading procedure for one time step in \textit{lemlab}}
    \label{fig:lem_structure}
\end{figure}

% case study/grids
\begin{figure}
    \centering
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/grid_countryside.pdf}
        \caption{Countryside}
    \end{subfigure}      
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/grid_rural.pdf}
        \caption{Rural}
    \end{subfigure}      
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/grid_suburban.pdf}
        \caption{Suburban}
    \end{subfigure}     
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/grid_urban.pdf}
        \caption{Urban}
    \end{subfigure}
    
    \caption[The case study regions with the underlying grid topologies and the supplied buildings.]{The case study regions with the underlying grid topologies and the supplied buildings. Each building may consist of multiple roof sections, each of which is represented as an individual polygon in the maps \cite{Candas2024}.}
    \label{fig:grid_topologies}
\end{figure}


==> source/SC_biblio.tex <==
      @article{TobiasLoga.2016,
 abstract = {In the framework of the international projects TABULA and EPISCOPE residential building typologies have been created in 20 European countries. Each national typology consists of a classification scheme grouping buildings according to their size, age and further parameters and a set of exemplary buildings representing these building types. U-values of different age bands and energy expenditure factors of heat generators of these buildings are being compared. In addition, synthetical average buildings have been defined which are statistically representative for specific age and size bands and enable projections of the energy performance to the total housing stocks. Based on the common data structure the energy performance of the average buildings is calculated in a standardised way to form simplified housing stock models. In the context of inhomogeneous building stocks of European countries the results allow an understanding of the average and variation of parameters like U-values, supply system performances or final energy.},
 author = {{Tobias Loga} and {Britta Stein} and {Nikolaus Diefenbach}},
 year = {2016},
 title = {{TABULA building typologies in 20 European countries—Making energy-related features of residential building stocks comparable}},
 url = {https://www.sciencedirect.com/science/article/pii/S0378778816305837},
 keywords = {Building stock models;Building typology;Calibration to measured consumption;EPISCOPE;Exemplary buildings;Nearly zero-energy buildings;Synthetical average buildings;TABULA;Webtool},
 pages = {4--12},
 volume = {132},
 issn = {0378-7788},
 journal = {{Energy and Buildings}},
 doi = {10.1016/j.enbuild.2016.06.094}
}

@misc{ArnoDentel.2006,
 author = {{Arno Dentel} and {Udo Dietrich}},
 date = {2006},
 title = {{Thermal comfort in buildings (Thermische Behaglichkeit - Komfort in Gebäuden)}},
 url = {https://rom-umwelt-stiftung.de/wp-content/uplo%ads/2006/02/Dokumentation_Thermische_Behaglichkeit.pdf},
 institution = {{HafenCity Universität Hamburg}}
}


@article{StefanPfenninger.2016,
 abstract = {Solar PV is rapidly growing globally, creating difficult questions around how to efficiently integrate it into national electricity grids. Its time-varying power output is difficult to model credibly because it depends on complex and variable weather systems, leading to difficulty in understanding its potential and limitations. We demonstrate how the MERRA and MERRA-2 global meteorological reanalyses as well as the Meteosat-based CM-SAF SARAH satellite dataset can be used to produce hourly PV simulations across Europe. To validate these simulations, we gather metered time series from more than 1000~PV systems as well as national aggregate output reported by transmission network operators. We find slightly better accuracy from satellite data, but greater stability from reanalysis data. We correct for systematic bias by matching our simulations to the mean bias in modeling individual sites, then examine the long-term patterns, variability and correlation with power demand across Europe, using thirty years of simulated outputs. The results quantify how the increasing deployment of PV substantially changes net power demand and affects system adequacy and ramping requirements, with heterogeneous impacts across different European countries. The simulation code and the hourly simulations for all European countries are available freely via an interactive web platform, www.renewables.ninja.},
 author = {{Stefan Pfenninger} and {Iain Staffell}},
 year = {2016},
 title = {{Long-term patterns of European PV output using 30 years of validated hourly reanalysis and satellite data}},
 url = {https://www.sciencedirect.com/science/article/pii/S0360544216311744},
 keywords = {Grid integration of renewables;Meteorological reanalysis;Renewables;Satellite irradiance estimation;Solar energy},
 pages = {1251--1265},
 volume = {114},
 issn = {03605442},
 journal = {{Energy}},
 doi = {10.1016/j.energy.2016.08.060}
}


@misc{ClaudiaNobis.2018,
 author = {{Claudia Nobis} and {Tobias Kuhnimhof}},
 date = {2018},
 title = {{Mobility in Germany - MiD result report (de: Mobilität in Deutschland - MiD Ergebnisbericht): (de: Studie von infas, DLR, IVT und infas 360 im Auftrag des Bundesministers für Verkehr und digitale Infrastruktur (FE-Nr. 70.904/15))}},
 url = {https://www.mobilitaet-in-deutschland.de/archive/pdf/MiD2017_Ergebnisbericht.pdf}
}



@article{GaeteMorales.2021,
 abstract = {There is substantial research interest in how future fleets of battery-electric vehicles will interact with the power sector. Various types of energy models~are used for respective analyses. They depend on meaningful input parameters, in particular time series of vehicle mobility, driving electricity consumption, grid availability, or grid electricity demand. As the availability of such data is highly limited, we introduce the open-source tool emobpy. Based on mobility statistics, physical properties of battery-electric vehicles, and other customizable assumptions, it derives time series data that can readily be used in a wide range of model applications. For an illustration, we create and characterize 200 vehicle profiles for Germany. Depending on the hour of the day, a fleet of one million vehicles has a median grid availability between 5 and 7 gigawatts, as vehicles are parking most of the time. Four exemplary grid electricity demand time series illustrate the smoothing effect of balanced charging strategies.},
 author = {Gaete-Morales, Carlos and Kramer, Hendrik and Schill, Wolf-Peter and Zerrahn, Alexander},
 year = {2021},
 title = {{An open tool for creating battery-electric vehicle time series from empirical data, emobpy}},
 pages = {152},
 volume = {8},
 number = {1},
 issn = {2052-4463},
 journal = {{Scientific Data}},
 doi = {10.1038/s41597-021-00932-9}
}
